A finite operator learning technique for mapping the elastic properties of microstructures to their mechanical deformations

To obtain fast solutions for governing physical equations in solid mechanics, we introduce a method that integrates the core ideas of the finite element method with physics-informed neural networks and concept of neural operators. This approach generalizes and enhances each method, learning the parametric solution for mechanical problems without relying on data from other resources (e.g. other numerical solvers). We propose directly utilizing the available discretized weak form in finite element packages to construct the loss functions algebraically, thereby demonstrating the ability to find solutions even in the presence of sharp discontinuities. Our focus is on micromechanics as an example, where knowledge of deformation and stress fields for a given heterogeneous microstructure is crucial for further design applications. The primary parameter under investigation is the Young's modulus distribution within the heterogeneous solid system. Our investigations reveal that physics-based training yields higher accuracy compared to purely data-driven approaches for unseen microstructures. Additionally, we offer two methods to directly improve the process of obtaining high-resolution solutions, avoiding the need to use basic interpolation techniques. First is based on an autoencoder approach to enhance the efficiency for calculation on high resolution grid point. Next, Fourier-based parametrization is utilized to address complex 2D and 3D problems in micromechanics. The latter idea aims to represent complex microstructures efficiently using Fourier coefficients. Comparisons with other well-known operator learning algorithms, further emphasize the advantages of the newly proposed method.

==> app.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Appendix A: basics of the continuum theory and finite element discretization}

The kinematic relation defines the strain tensor $\bm{\varepsilon}$ in terms of the deformation vector $\bm{U}^T=[U,~ V]$ and reads:
\begin{align}
\label{kinematics}
\bm{\varepsilon}\,=\,\text{sym}(\text{grad}(\bm{U})) = \nabla^s\bm{U} = \dfrac{1}{2}\left(\nabla \bm{U} + \nabla \bm{U}^T \right).
\end{align} 
In the context of linear elasticity, we define the elastic energy of the solid as 
\begin{align}
\label{lin_energy}  
\psi_{lin} = \dfrac{1}{2}~\bm{\varepsilon}:\mathbb{C}(\bm{X}):\bm{\varepsilon},
\end{align}
where $\mathbb{C}$ is the fourth-order elasticity tensor. Through the constitutive relation, one relates the stress tensor to the strain tensor via 
\begin{align}
\label{materiallaw4}  
{\bm{\sigma}} &= {\mathbb{C}}(\bm{X})~{\bm{\varepsilon}}, \\
\mathbb{C}(\bm{X}) &= \Lambda(\bm{X})~\mathbf{I} \otimes \mathbf{I} + 2\mu(\bm{X})~\mathbb{I}^s.
\end{align}
Defining $\mathbf{I}$ as the second-order identity tensor and $\mathbb{I}^s$ as the symmetric fourth-order identity tensor, the above relation can also be written in the following form
\begin{align}
\label{materiallaw_Lamme}  
\boldsymbol{\sigma} = \Lambda(\bm{X}) \, \text{tr}(\boldsymbol{\varepsilon}) \, \mathbf{I} + 2\mu(\bm{X}) \, \boldsymbol{\varepsilon}.
\end{align}
Here, we have position-dependent Lame constants which can be written in terms of Young modulus $E$ and Poisson ratio $\nu$ as $\Lambda=E\nu/[(1-2\nu)(1+\nu)]$ and $\mu= E/[2(1+\nu)]$.
Here, the elastic properties are phase-dependent and vary throughout the microstructure. Finally, the mechanical equilibrium in the absence of body force, as well as the Dirichlet and Neumann boundary conditions, are written as:
\begin{align}
\label{Equilbrium}
\text{div}({\bm{\sigma}}) = \text{div}(\mathbb{C}(\bm{X})\nabla^s\bm{U})\ &= \bm{0}~~~~\text{in}~~~ \Omega\\
\label{BcsMech_d}
\bm{U} &= \bar{\bm{U}}~~~\text{on}~~\Gamma_D \\ 
\label{BcsMech_n}
\bm{\sigma} \cdot \bm{n} = \bm{t} &= \bar{\bm{t}}~~~~\text{on}~~\Gamma_N
\end{align} 
In the above relations, $\Omega$ and $\Gamma$ denote the material points in the body and on the boundary area, respectively. Moreover, the Dirichlet and Neumann boundary conditions are introduced in Eq.~\ref{BcsMech_d} and Eq.~\ref{BcsMech_n}, respectively.
Rewriting Eq.~\ref{materiallaw4} in the Voigt notation, we have $\hat{\bm{\sigma}}=\boldsymbol C(\bm{X})\hat{\bm{\varepsilon}}$. Considering the plane stress assumption in 2D, we write:
\begin{align}
\label{elasticityPlanestrain}
\boldsymbol C(\bm{X})\,=\, \dfrac{E(\bm{X})}{1-\nu^2(\bm{X})}\,\begin{bmatrix} 1 & \nu(\bm{X}) & 0 \\
\nu(\bm{X}) & 1 & 0 \\
0 & 0 & \dfrac{1-\nu(\bm{X})}{2}
\end{bmatrix}.
\end{align}
It is assumed that the material behavior remains isotropic in each phase. 

By introducing $\delta\bm{U}^T=[\delta U,~\delta V]$ as standard test functions and performing integration by parts, the weak form of the mechanical equilibrium problem reads:
\begin{align}
\label{Weakform}
\int_{\Omega} \delta{\bm{\hat{\varepsilon}}}^T\,\boldsymbol C(\bm{X})\,\hat{\bm{\varepsilon}}\,~dV\,-\, \int_{\Gamma_N} \delta{\bm{U}^T}\,\bar{\bm{t}}~dA=0. 
\end{align} 
The weak form in Eq.~\ref{Weakform} can also be interpreted as the balance between the mechanical internal energy $E^M_{\text{int}}$ and mechanical external energy $E^M_{\text{ext}}$. 

Next, we shortly summarize the corresponding linear shape functions $\bm{N}$ and the deformation matrix $\bm{B}$ used to discretize the mechanical weak form in the current work.
\begin{align}
\label{eq:N}
\bm{N} =
\begin{bmatrix}
N_1 & 0 & \dots & N_4 & 0\\
0 & N_1 & \dots & 0 & N_4
\end{bmatrix},~
\bm{B} =
\begin{bmatrix}
N_{1,x} & 0       & \dots & N_{4,x} & 0        \\
0       & N_{1,y} & \dots & 0       & N_{4,y}  \\
N_{1,y} & N_{1,x} & \dots & N_{4,y} & N_{4,x} 
\end{bmatrix}.
\end{align}
The notation $N_{i,x}$ and $N_{i,y}$ represent the derivatives of the shape function $N_i$ with respect to the coordinates $x$ and $y$, respectively. To compute these derivatives, we utilize the Jacobian matrix
\begin{align}
 \boldsymbol J = \partial \boldsymbol X / \partial \boldsymbol \xi = \begin{bmatrix} \frac{\partial x}{\partial \xi} & \frac{\partial y}{\partial \xi} \\ \frac{\partial x}{\partial \eta} & \frac{\partial y}{\partial \eta} \end{bmatrix}. 
\end{align}

Here, $\boldsymbol X = [x, y]$ and $\boldsymbol \xi = [\xi, \eta]$ represent the physical and parent coordinate systems, respectively. It is worth mentioning that this determinant remains constant for parallelogram-shaped elements, eliminating the need to evaluate this term at each integration point.
Readers are also encouraged to see the standard procedure in any finite element subroutine \cite{bathe, hughes}.
Finally, for the B matrix, we have 
\begin{align}
 \bm{B} = \bm{J}^{-1} \begin{bmatrix} \frac{\partial N_1}{\partial \xi} & 0 & \frac{\partial N_2}{\partial \xi} & 0 & \frac{\partial N_3}{\partial \xi} & 0 & \frac{\partial N_4}{\partial \xi} & 0 \\ 0 & \frac{\partial N_1}{\partial \eta} & 0 & \frac{\partial N_2}{\partial \eta} & 0 & \frac{\partial N_3}{\partial \eta} & 0 & \frac{\partial N_4}{\partial \eta} \\ \frac{\partial N_1}{\partial \eta} & \frac{\partial N_1}{\partial \xi} & \frac{\partial N_2}{\partial \eta} & \frac{\partial N_2}{\partial \xi} & \frac{\partial N_3}{\partial \eta} & \frac{\partial N_3}{\partial \xi} & \frac{\partial N_4}{\partial \eta} & \frac{\partial N_4}{\partial \xi} \end{bmatrix}. 
\end{align}


\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/FE_int.jpg}
  \caption{The physical space and the parent space. Gaussian integration and shape functions are shown specifically within the parent space. }
  \label{fig:FE_int}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
\color{black}


%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Appendix B: More details on the training of the DeepONet part}
In this appendix, additional details about the training process of the DeepONet network are provided.
Sec.\,\ref{DeepONet} illustrates the vanilla DeepONet network architecture in Fig.\,
\ref{fig:DNOarch}.
The branch network processes the distribution of properties, which are measured at arbitrary sensor locations. Specifically, the input function to the branch network includes the values of Young's modulus at the element nodes. The branch maps the input function into two distinct vectors, one for each output. They can be considered as latent vectors, see \cite{boulle2023}. On the other hand, the trunk network is designed to receive the spatial coordinates of a single point where the output function is evaluated. Finally, two operators are built by the dot product of the last layers of the branch and the trunk. 

These operators are designed to map the input function $\bm{E}$, captured at $N$ sensor locations (nodes of elements), to the corresponding solutions at the given spatial coordinate $\bm{X}=(x_i, y_i)$ to the trunk network. 

In Eq.~\ref{eq:deeponetloss}, the loss function is defined as the mean squared error (MSE) between the predicted values of the operators for $U$ and $V$ and the solutions derived using the finite element method (FEM). For each input function, indexed by $i$ and covering the entire range of training inputs up to $I_{train}$, the total number of training input functions, the operator predicts the value at each point $j$. Then the difference between these predictions and the solutions obtained by FEM over $N$ points are computed. The network parameters, denoted as $\bm{\theta}$, are then optimized by minimizing the loss function outlined in Eq.~\ref{eq:deeponetloss}. 

For training the network, a purely data-driven approach is employed. Details regarding the sample preparation can be found in Sec.\,\ref{preparationofcollocationfields}. The training involves $4000$ samples, each featuring distinct morphology maps, and the training is done for $4000$ epochs. Since the architecture of the network differs significantly from the FOL approach, an extensive study of hyperparameters was performed to achieve optimal results. The best-performing configuration was found to be $6[20]$, which indicates $6$ hidden layers when each layer consists of $20$ neurons. Notably, both the branch and the trunk networks use an identical architecture and share a common final layer containing $20$ neurons.
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.50\linewidth]{./Figs/dno_loss.pdf}
  \caption{The decay of total loss and its $U$ and $V$ components for the DeepONet network with optimally found hyperparameters.}
  \label{fig:dno_loss}
\end{figure}
The best result is obtained by using the \emph{swish} as the activation function. The loss decay for the optimal hyperparameters is shown in Fig.\,\ref{fig:dno_loss}.



\color{blue}

%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Appendix C: Supplementary results}

\begin{figure}[H] 
  \centering
  \includegraphics[width=1.0\linewidth]{./Figs/test0.jpg}
  \caption{Predictions of the trained FOL for a test case with three square shape inclusions.}
  \label{fig:test0}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=1.0\linewidth]{./Figs/test2.jpg}
  \caption{Predictions of the trained FOL for test similar to architectured materials which behave anisotropic.}
  \label{fig:test2}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/FOL_conv_DD_2.jpg}
  \caption{Performance of data-driven and physics-driven approaches for the different number of training samples.
   }
  \label{fig:FOL_conv_DD_2}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.95\linewidth]{./Figs/MEA_res.jpg}
  \caption{ MEA Mech results (displacement component $U$). }
  \label{fig:MEA_res}
\end{figure}

\color{black}

==> draft.tex <==
%\begin{align}
%\frac{\partial N_1}{\partial \xi} &= -\frac{1}{4}(1 - \eta), & \frac{\partial N_1}{\partial \eta} &= -\frac{1}{4}(1 - \xi), \
%\frac{\partial N_2}{\partial \xi} &= \frac{1}{4}(1 - \eta), & \frac{\partial N_2}{\partial \eta} &= -\frac{1}{4}(1 + \xi), \
%\frac{\partial N_3}{\partial \xi} &= \frac{1}{4}(1 + \eta), & \frac{\partial N_3}{\partial \eta} &= \frac{1}{4}(1 + \xi), \
%\frac{\partial N_4}{\partial \xi} &= -\frac{1}{4}(1 + \eta), & \frac{\partial N_4}{\partial \eta} &= \frac{1}{4}(1 - \xi).
%\end{align}

% 
%Next, we review the finite element implementation of the model. The weak form is constructed by multiplying the equations in Eq. \ref{eq:strong form govering equations}(a-c) by a corresponding arbitrary test function and integrating them over the domain of the problem. With integration by parts, the corresponding weak forms are:
%\begin{align}
%\int_{\Omega}k\nabla T \nabla \delta_{T}dV -\int_{\Omega_t}k\nabla T \delta_{T}dS +\int_{\Omega}\rho {c}\dot{T}\delta_{T}dV-\int_{\Omega}Q\delta_{T}dV=0.
%\end{align} 
%\label{eq:weak_form}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/NN_FE.jpg}
  \caption{ Network architecture and loss functions for the COMM-PINN applied to interface failure with nonlinear softening law. }
  \label{fig:NN_FE}
\end{figure}

%\begin{align}
%\label{eq:dis_residual}
%\boldsymbol r_{T}=&\int_{\Omega} [\boldsymbol  B_{T}]^T k\boldsymbol  B_{T} dV-\int_{\Omega_t}[\boldsymbol  B_{T}]^T k\boldsymbol  N_{T}dS +\int_{\Omega}\rho c \dot T [\boldsymbol  N_{T}]dV-\int_{\Omega} [\boldsymbol  N_{T}]^TQdV. 
%\end{align}

\begin{algorithm}[H]
\caption{Solving the damage governing equations at pseudo time $t^{i+1}$}
\label{alg:dmg}
\begin{algorithmic}[1]
\item[\textbf{Input:}] interface's parameters, current gap: ${g}^{i+1}$, history variables: $d^i$, $\xi^i_d$
\item[\textbf{Output:}] current traction: ${T}^{i+1}$, current history variables $d^{i+1}$, $\xi_d^{i+1}$, tangent: ${C}_d=\text{d} {T}^{i+1} / \text{d} {g}^{i+1}$
\State $k=1$
\State Set trial values: ${g}^k_p={g}^{i}_p$, $d^k=\xi^{i}_d=d^i$
\State \textbf{loop} \textit{damage solver} \textbf{do} \\
\vspace{1mm}
$\qquad $ \textbf{if} $\phi^{tr}_d = {K} (g^{i+1})^2 - \left( Y_{0} + q_d(\xi^{i}) \right) \le 0$ \\
\vspace{1mm}
$\qquad $ $\qquad $   $d^{i+1}=d^{i}$, $\xi^{i+1}_d=\xi^{i}_d$ and ${C}_d=(1-d^{i+1})^2K $ \\ 
\vspace{1mm}
$\qquad $ \textbf{else} solve for $d^{k+1}$ and $\xi^{k+1}_d = \xi^{i}_d+\Delta \lambda^{k+1}_d$ (see Eqs~\ref{eq:dm_y},\ref{eq:dmg_ev})\\
\vspace{1mm}
$\qquad $  $\qquad  r^{(1)}_d = d^{k+1} - d^i - (\xi^{k+1}_d - \xi^{i}_d) \dfrac{\partial \phi_d}{\partial Y} \stackrel{!}{=} 0$ \\
$\qquad $  $\qquad  r^{(2)}_d = \phi_d = Y - \left( Y_{0} + q_d\left( \xi^{i+1}_d \right) \right) \stackrel{!}{=} 0$ \\
\vspace{1mm}
$\qquad$  $\qquad [d^{i+1,k+1}~~~ \xi^{i+1,k+1}_d]^T = [d^{i+1,k}~~~\xi^{i+1,k}_d]^T - \boldsymbol{K}_d^{-1} \boldsymbol{r}_d$ \\
%$\qquad $  $\qquad  $ Update the values of $d^{k+1}$, $\xi^{k+1}_d$ \\
$\qquad $ \textbf{end if} \\
\vspace{1mm}
$\qquad $ \textbf{if} $\left| {d}^{i+1,k+1}-{d}^{i+1,k}\right|>\text{tol} $ \textbf{OR} $\left| \xi^{i+1,k+1}_d-\xi^{i+1,k}_d\right|>\text{tol}$ \\
$\qquad $ $\qquad $   $k++$ \\
$\qquad $ $\qquad $   \textbf{CYCLE loop} \textit{damage solver} \\ 
$\qquad $ \textbf{else} \\
$\qquad $ $\qquad $  $d^{i+1}=d^{i+1,k+1}$, $\xi^{i+1}_d=\xi^{i+1,k+1}_d$ \\
\vspace{1mm}
$\qquad $ $\qquad $   \textbf{EXIT loop} \textit{damage solver} \\
$\qquad $ \textbf{end if}
\vspace{1mm}
\State \textbf{end loop}
\State Compute traction ${T}=(1-d^{i+1})^2 {K} {g}^{i+1}$
\State Compute tangent ${C}_d $ 
\end{algorithmic}
\end{algorithm}

\begin{align}
N_1 = \frac{1}{4} (1 - \xi) (1 - \eta),~
N_2= \frac{1}{4} (1 + \xi) (1 - \eta),~
N_3 = \frac{1}{4} (1 + \xi) (1 + \eta),~
N_4 = \frac{1}{4} (1 - \xi) (1 + \eta)
\end{align}


\begin{align}
\label{loss_ene}
\mathcal{L}_{ene} &= \text{MSE}\left( (d^{i+1}-d^{i})\text{Relu}(-\phi^{tr}_d) \right), \\
\label{loss_bcs}
\mathcal{L}_{dbc} &= \text{MSE}\left( (\xi^{i+1}_d-\xi^{i}_d)\text{Relu}(-\phi^{tr}_d) \right).
\end{align}

The mean squared error is defined as
\begin{align}
\label{eq:MSE}
\text{MSE}( \bullet )_{type} &= \dfrac{1}{n}\sum_{i=1}^{n}(\bullet)^2, 
\end{align}
where $n$ is the number of observation points. 




\begin{align}
\label{Totalloss}
\mathcal{L}_{tot} =  
\underbrace{
\sum_{e=1}^{n_{el}}\boldsymbol T^T_e \left[ \boldsymbol \sum_{n=1}^{n_{int}} \dfrac{w_n}{2}~\text{det}(\boldsymbol J)~\boldsymbol B_{T}^T [\boldsymbol C_e] \boldsymbol B_{T} \right] \boldsymbol T_e 
}_{\text{energy + Neumann BCs}} 
+
\quad \lambda_b\underbrace{\sum_{i=1}^{n_{db}} \mathcal{L}_{db,i}}_{\text{Drichlet BCs}} 
\end{align}


The creation of sample are described in Alg.~\ref{alg:sample}.
\begin{algorithm}[H]
\caption{Collocation point generation for solving the interface damage model}
\label{alg:sample}
\begin{algorithmic}[1]
\item[\textbf{Input:}] step size: $st$, begin $bg$ and end of interval $en$, $n=1$
\item[\textbf{Output:}] admissible set of inputs for training $\bold{IN}_d$
\State Initializing: $\boldsymbol{g}=[bg_{g}:st_{g}:en_{g}]$, $\boldsymbol{d}=[bg_{d}:st_{d}:en_{d}]$, $\boldsymbol{\xi}_d=[bg_{\xi_d}:st_{\xi_d}:en_{\xi_d}]$
\State \textbf{for} l \textbf{in} $\boldsymbol{g}$ \textbf{do} \\
\vspace{1mm}
$\qquad $ \textbf{for} j \textbf{in} $\boldsymbol{d}$ \textbf{do} \\
\vspace{1mm}
$\qquad $ $\qquad $ \textbf{for} k \textbf{in} $\boldsymbol{\xi_d}$ \textbf{do} \\ 
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad $ $\bold{IN}_d[n,1]$ = $\boldsymbol{g}[l]$\\
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad $ $\bold{IN}_d[n,2]$ = $\boldsymbol{d}[j]$\\
\vspace{1mm}
$\qquad$ $\qquad$ $\qquad$ \textbf{if} $\boldsymbol{\xi}_d[k] = \boldsymbol{d}[j]$  \\
\vspace{1mm}
$\qquad $ $\qquad$ $\qquad$ $\qquad$ $\bold{IN}_d[n,3]$ = $\boldsymbol{\xi}_d[k]$\\
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad$ $\qquad$ $n++$\\
$\qquad $ $\qquad $ $\qquad$ \textbf{end if}
\end{algorithmic}
\end{algorithm}


\begin{align}
\label{int_Energy}
\text{Minimize:~}&\underbrace{\int_{\Omega}\dfrac{1}{2}\hat{\bm{\varepsilon}}^T\,\hat{{{C}}}(x,y)\,\hat{\bm{\varepsilon}}\,~dV}_{E^M_{\text{int}}} - 
\underbrace{\int_{\Gamma_N} {\bm{u}^T}\,\bar{\bm{t}}~dA}_{E^M_{\text{ext}}},\\
\label{int_Energy_bcs}
\text{Subjected to:~}& \text{BCs in Eq.~\ref{BcsMech_d} and Eq.~\ref{BcsMech_n}}.
\end{align}
The expressions in Eqs.~\ref{int_Energy} and \ref{int_Energy_bcs} will be added directly to the loss function of the neural network for the primary variable $\bm{u}$ (see also \cite{SAMANIEGO2020112790}).

%\begin{align}
%\label{materiallaw}
%\hat{\bm{\sigma}}\,=\hat{{C}}(x,y)~\hat{\bm{\varepsilon}}.
%\end{align} 
%In Eq.~\ref{materiallaw}, $\hat{\bullet}$ denotes the tensor ($\bullet$) in the Voigt notation. 
% To obtain the Galerkin weak form (WF) of the problem we first multiply Eq.~\ref{Equilbrium} by a test function $\delta \bm{u}$ of the given boundary value problem. By applying integration by parts and utilizing Gauss theorem one obtains


%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Influence of the number of training samples}
In Figures \ref{fig:SN_1} and \ref{fig:SN_2}, we analyze the impact of the number of initial sample fields. In the selected 2000 samples, we excluded mainly morphologies with ring shape. For the depicted test cases, we observed a reduction in the maximum difference by a factor of 2.0 and 1.6. This suggests that enhancing the quantity and diversity of initial random fields can improve the quality of results for unseen test cases. Notably, the training cost did not notably increase as we doubled the batch size while increasing the number of samples.
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/SN_1.jpg}
  \caption{Influence of the initial training fields for the introduced physics-informed deep learning model (FOL).}
  \label{fig:SN_1}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/SN_2.jpg}
  \caption{Influence of the initial training fields for the introduced physics-informed deep learning model (FOL).}
  \label{fig:SN_2}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Influence of activation functions}
In Fig.~\ref{fig:af}, we look into the influence of various choices for the activation function on the predictions. To avoid repetition, only the pointwise error for each choice of the activation function is shown in each row and column of Fig.~\ref{fig:af}. Except for the linear case, which is an oversimplified case, the errors using other types of activation functions remain low.
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/af.jpg}
  \caption{Influence of the type of activation functions on the obtained results.}
  \label{fig:af}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.8\linewidth]{./Figs/err.jpg}
  \caption{ Evaluation of averaged errors for different choice of activation functions. }
  \label{fig:err}
\end{figure}


%%%% HERE
In total, the tanh and swish functions showed the best performance. For a better and more quantitative comparison, the cross-section of the predictions and averaged errors are reported in Fig.~\ref{fig:err}. To avoid repetition, the error values in this case are calculated based on $Err = \frac{| \langle T_{NN} \rangle - \langle T_{FE} \rangle|}{| \langle T_{FE} \rangle|}\times 100$, where we have $\langle T_{NN} \rangle = \frac{1}{N^2}\Sigma_i T_{NN}(i)$. This is motivated by the idea of homogenization, where we average the obtained temperature and heat flux to obtain the overall material properties. The lower this homogenized error is, the higher the accuracy will be for the homogenization of properties

Interestingly, the errors for the homogenized temperature are below $1\%$, which also holds for many other test cases not reported here. On the other hand, the average error for the flux in x-direction is higher, which is reasonable since we only predict the temperature profile and any slight fluctuations in the predicted temperature influence its spatial derivatives. The errors for the heat flux using the swish option are still acceptable and remain between $2\%$ to $3\%$. One should note that ideas from mixed formulations, where we predict the heat flux as an output, can also be integrated with the current formulation to enhance the predictive ability of the neural network for higher-order gradients of the solutions (see investigations in \cite{REZAEI2022PINN, Faroughi2023}).

%%%%%%%%%%%%%%%%%%%%%%%%%%5
%\newpage%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Influence of the network architecture}
As discussed in the previous section, the NN architecture is designed to relate all the inputs to one single output. As a result, we are dealing with a parallel series of networks that initially act independently and then are connected through the physics-based loss functions. In this section, we emphasize the importance of this approach by evaluating and training the very same network architecture where we have a fully connected network to map the whole input to the whole output. The number of layers and neurons in each are set to obtain the same numbers from the previous case to ensure a fair comparison. Therefore, we still have 2 layers but with $10 \times 121 = 1210$ neurons in each. The predictions are reported in Fig.~\ref{fig:NN_arch}, where we observe very high errors and rather poor performance from the NN.
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/NN_arch.jpg}
  \caption{Poor performance of the network by using standard fully connected neural nets instead of separating them. The network parameters such as number of neurons and layers are kept the same as before.}
  \label{fig:NN_arch}
\end{figure}
It is worth mentioning that the network in this case simply captures the dominant solution, which is a rather linear distribution of temperature from left to right without being able to capture the influence of introduced heterogeneity. Keep in mind that other hyperparameters are also set as before, and even upon changing them for better results, we did not find significant improvements through further parameter studies.


%As anticipated from Fig.~\ref{fig:loss}, the NN's outcomes are unreliable before 1000 epochs. Surprisingly, after 1000 epochs, the NN demonstrates an acceptable level of training. However, continuing the training up to 4000 epochs improved the overall results. It is noteworthy that the results showcased in Figures \ref{fig:evol_1} correspond to test cases where these morphologies were unseen by the NN. Similar trends were observed for other test cases within or outside the training set, although not presented here to maintain conciseness in the results section. More comprehensive comparisons and quantitative error analyses are provided in subsequent sections.
%\\ \\
%\textbf{Remark 4} Rather than relying on finite element interpolation functions, which do not add any additional information and merely smooth the results, an alternative approach involves employing a pre-trained decoder network. This network can map the solution space from a coarse grid to a finer grid. Similar ideas have been explored in \cite{kontolati2023learning}.
%\\ \\
%\textbf{Remark 5} We exclusively predict temperature profiles in the current approach. Consequently, the flux vector, as presented in subsequent studies, is derived via local numerical differentiation of the temperature. However, an extension of this approach could involve a mixed formulation, predicting the flux values as additional outputs for the network to further enhance predictions, as explored in works such as \cite{Faroughi22, REZAEI2022PINN, Harandi2023}.


\begin{align}
\label{elasticityPlanestrain}
\boldsymbol C(\bm{X})\,=\, \dfrac{E(\bm{X})}{(1-2\nu(\bm{X}))(1+\nu(\bm{X}))}\,\begin{bmatrix} 1-\nu(\bm{X}) & \nu(\bm{X}) & 0 \\
\nu(\bm{X}) & 1-\nu(\bm{X}) & 0 \\
0 & 0 & \dfrac{1-2\nu(\bm{X})}{2}
\end{bmatrix}.
\end{align}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.8\linewidth]{./Figs/cross_plot_1.jpg}
  \caption{Comparison of data-driven and physics-driven approaches regarding the temperature and flux profiles. \textcolor{red}{lets add DeepOnet to it... better color choice and omit legends... smooth the results? } }
  \label{fig:cross_plot}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.8\linewidth]{./Figs/cross_plot_2.jpg}
  \caption{Comparison of data-driven and physics-driven approaches regarding the temperature and flux profiles. \textcolor{red}{lets add DeepOnet to it... better color choice and omit legends... smooth the results? } }
  \label{fig:cross_plot}
\end{figure}


\begin{table}[H]
\fontsize{7}{10}\selectfont
\centering
\caption{ Comparison of different approaches for solving PDEs.}
\label{tab:compare} \begin{adjustbox}{center}
\begin{tabular}{ l l l l }
\hline
---   &  FEM  & PINN &  FOL  \\
\hline
Implementing/Transferring codes  &  Hard (software specific)  & Easy (only network evaluation) & Easy (only network evaluation)  \\
Training time  &   - (doesn't apply)  & Moderate-high (based on AD) & Moderate (based on shape functions) \\
Parametric learning  &  No  & Yes (upon using extra inputs or branch net) & Yes \\
Order of derivations  &  Low (weak form)  & High (unless using DEM or Mixed-PINN) & Low (weak form)  \\
Handling complex geometries  &  Yes  & Yes & Yes \\
Handling strong heterogeneity  &  Yes  & Yes, by using Mixed PINN or domain decomp. & Yes \\
Data requirement  &  Only model param.  & Only model param. & Only model param.  \\ 
&  & no additional solution is required & no additional solution is required \\
\hline
Main limitation  &  Comput. cost + Discretization error  & Training cost + Training range & Training range + Discretization error  \\
Main advantage  &   Accurate solutions for various PDEs  & Fast eval. + No data is required & Fast eval. + No data is required \\
\hline
\end{tabular}
\end{adjustbox}{}
\end{table}



\textcolor{purple}{I think the interpolation approach would be a questionable approach for many reviewers, as I feel that in your previous paragraph you tried to indirectly show the benefits of the interpolation approach by discussing the training loss of MEA. I think it would be safer if you did not support this approach, because if it was so great, it would be implemented by many commercial FE software companies. If you want to look at your model as a generalized model in many domains, then the interpolation model would be scary because it doesn't capture the sharp interfaces at least in fluied mechanics where the interfaces are very important. For FE2 models, however, it would be an advantage. So BE CAREFUL!}


%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.60\linewidth]{./Figs/ff_12_u.png}
  \caption{ res. }
  \label{fig:ff_12_u}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.60\linewidth]{./Figs/ff_12_s.png}
  \caption{ res. }
  \label{fig:ff_12_s}
\end{figure}


\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./Figs/ff_10_u.png}
        \label{fig:subplot1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./Figs/ff_10_s.png}
        \label{fig:subplot2}
    \end{subfigure}
    \caption{Main caption for both images}
    \label{fig:main}
\end{figure}


\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./Figs/ff_12_u.png}
        \label{fig:subplot1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./Figs/ff_12_s.png}
        \label{fig:subplot2}
    \end{subfigure}
    \caption{Main caption for both images}
    \label{fig:main}
\end{figure}
